Learning of Structurally Unambiguous Probabilistic Grammars

The problem of identifying a probabilistic context free grammar has two aspects: the first is determining the grammar's topology (the rules of the grammar) and the second is estimating probabilistic weights for each rule. Given the hardness results for learning context-free grammars in general, and probabilistic grammars in particular, most of the literature has concentrated on the second problem. In this work we address the first problem. We restrict attention to structurally unambiguous weighted context-free grammars (SUWCFG) and provide a query learning algorithm for structurally unambiguous probabilistic context-free grammars (SUPCFG). We show that SUWCFG can be represented using co-linear multiplicity tree automata (CMTA), and provide a polynomial learning algorithm that learns CMTAs. We show that the learned CMTA can be converted into a probabilistic grammar, thus providing a complete algorithm for learning a structurally unambiguous probabilistic context free grammar (both the grammar topology and the probabilistic weights) using structured membership queries and structured equivalence queries. We demonstrate the usefulness of our algorithm in learning PCFGs over genomic data.

==> algorithm.tex <==
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
%\usepackage{algpseudocode}
%\usepackage[ruled, vlined, linesnumbered]{algorithm2e}

\algrenewcommand\alglinenumber[1]{{\footnotesize#1}}
\algrenewcommand\algorithmicrequire{\textbf{Precondition:}}
\algrenewcommand\algorithmicensure{\textbf{Postcondition:}}
\algnewcommand\Not[1]{\textbf{not} #1}
\algnewcommand\Continue{\textbf{continue}}
\algnewcommand\Break{\textbf{break}}

\newcommand*\Let[2]{\State #1 $\gets$ #2}
\newcommand{\Push}[2]{\Let{#1}{#1 $\cup$ #2}}
\newcommand{\Enqueue}[2]{\Let{#1}{#2 $\cup$ #1}}

% begin vertical rule patch for algorithmicx
% borrowing from https://tex.stackexchange.com/questions/41956/marking-conditional-versions-with-line-in-margin

\RequirePackage{tikz}
\RequirePackage{zref-abspage}
\RequirePackage{zref-user}
\RequirePackage{tikz}
\RequirePackage{atbegshi}
\usetikzlibrary{calc}
\RequirePackage{tikzpagenodes}
\RequirePackage{etoolbox}

\makeatletter
\newcommand*\ALG@lastblockb{b}
\newcommand*\ALG@lastblocke{e}
\apptocmd{\ALG@beginblock}{%
    %\typeout{beginning block, nesting level \theALG@nested, line \arabic{ALG@line}}%
    \ifx\ALG@lastblock\ALG@lastblockb
        \ifnum\theALG@nested>1\relax\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi{\ALG@tikzborder}{}%
    \fi
    \let\ALG@lastblock\ALG@lastblockb%
}{}{\errmessage{failed to patch}}

\pretocmd{\ALG@endblock}{%
    %\typeout{ending block, nesting level \theALG@nested, line \arabic{ALG@line}}%
    \ifx\ALG@lastblock\ALG@lastblocke
        \addtocounter{ALG@nested}{1}%
        \addtolength\ALG@tlm{\csname ALG@ind@\theALG@nested\endcsname}%
        \ifnum\theALG@nested>1\relax\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi{\endALG@tikzborder}{}%
        \addtolength\ALG@tlm{-\csname ALG@ind@\theALG@nested\endcsname}%
        \addtocounter{ALG@nested}{-1}%
    \fi
    \let\ALG@lastblock\ALG@lastblocke%
}{}{\errmessage{failed to patch}}


\tikzset{ALG@tikzborder/.style={line width=0.5pt,black}}

\newcommand*\currenttextarea{current page text area}

\newcommand*{\updatecurrenttextarea}{%
    \if@twocolumn
        \if@firstcolumn
            \renewcommand*{\currenttextarea}{current page column 1 area}%
        \else
            \renewcommand*{\currenttextarea}{current page column 2 area}%
        \fi
    \else
        \renewcommand*\currenttextarea{current page text area}%
    \fi
}


\newcounter{ALG@tikzborder}
\newcounter{ALG@totaltikzborder}
\newenvironment{ALG@tikzborder}[1][]{%
    % Allow user to overwrite the used style locally
    \ifx&#1&\else
        \tikzset{ALG@tikzborder/.style={#1}}%
    \fi
    \stepcounter{ALG@totaltikzborder}%
    \expandafter\edef\csname ALG@ind@border@\theALG@nested\endcsname{\theALG@totaltikzborder}%
    \setcounter{ALG@tikzborder}{\csname ALG@ind@border@\theALG@nested\endcsname}%
    %\typeout{begin ALG border nesting level=\theALG@nested, tikzborder=\theALG@tikzborder, tlm=\the\ALG@tlm}%
    \tikz[overlay,remember picture] \coordinate (ALG@tikzborder-\theALG@tikzborder);% node {\theALG@tikzborder};% Modified \tikzmark macro
    \zlabel{ALG@tikzborder-begin-\theALG@tikzborder}%
    % Test if end-label is at the same page and draw first half of border if not, from start place to the end of the page
    \ifnum\zref@extract{ALG@tikzborder-begin-\theALG@tikzborder}{abspage}=\zref@extract{ALG@tikzborder-end-\theALG@tikzborder}{abspage} \else
        \updatecurrenttextarea
        \ALG@drawvline{[shift={(0pt,.5\ht\strutbox)}]ALG@tikzborder-\theALG@tikzborder}{\currenttextarea.south east}{\ALG@thistlm}%
        % If it spreads over more than two pages:
        \newcounter{ALG@tikzborderpages\theALG@tikzborder}%
        \setcounter{ALG@tikzborderpages\theALG@tikzborder}{\numexpr-\zref@extract{ALG@tikzborder-begin-\theALG@tikzborder}{abspage}+\zref@extract{ALG@tikzborder-end-\theALG@tikzborder}{abspage}}%
        \ifnum\value{ALG@tikzborderpages\theALG@tikzborder}>1
            \edef\nextcmd{\noexpand\AtBeginShipoutNext{\noexpand\ALG@tikzborderpage{\theALG@tikzborder}{\the\ALG@thistlm}}}%some pages need a border on the whole page
            \nextcmd
        \fi
    \fi
}{%
    \setcounter{ALG@tikzborder}{\csname ALG@ind@border@\theALG@nested\endcsname}%
    %\typeout{end ALG border nesting level=\theALG@nested, tikzborder=\theALG@tikzborder, tlm=\the\ALG@tlm}%
    \tikz[overlay,remember picture] \coordinate (ALG@tikzborder-end-\theALG@tikzborder);% node {\theALG@tikzborder};% Modified \tikzmark macro
    \zlabel{ALG@tikzborder-end-\theALG@tikzborder}%
    % Test if begin-label is at the same page and draw whole border if so, from start place to end place
    \updatecurrenttextarea
    \ifnum\zref@extract{ALG@tikzborder-begin-\theALG@tikzborder}{abspage}=\zref@extract{ALG@tikzborder-end-\theALG@tikzborder}{abspage}\relax
        \ALG@drawvline{[shift={(0pt,.5\ht\strutbox)}]ALG@tikzborder-\theALG@tikzborder}{ALG@tikzborder-end-\theALG@tikzborder}{\ALG@thistlm}%
    % Otherwise draw second half of border, from the top of the page to the end place
    \else
        %\settextarea
        \ALG@drawvline{\currenttextarea.north west}{ALG@tikzborder-end-\theALG@tikzborder}{\ALG@thistlm}%
    \fi
}

\newcommand*{\ALG@drawvline}[3]{%#1=from, #2=to, #3=value of \ALG@tlm/\ALG@thisthm
    \begin{tikzpicture}[overlay,remember picture]
        \draw [ALG@tikzborder]
            let \p0 = (\currenttextarea.north west), \p1=(#1), \p2 = (#2)
             in
            (#3+\fboxsep+.5\pgflinewidth+\x0,\y1+\fboxsep+.5\pgflinewidth)%-\fboxsep-.5\pgflinewidth
             --
            (#3+\fboxsep+.5\pgflinewidth+\x0,\y2-\fboxsep-.5\pgflinewidth)
            %node[midway,anchor=east] {\ALG@tikzbordertext}
        ;
    \end{tikzpicture}%
}

\newcommand{\ALG@tikzborderpage}[2]{%the whole page gets a border, #1=value of \theALG@tikzborder, #2=value of \ALG@tlm/\ALG@thistlm
    \updatecurrenttextarea
    \setcounter{ALG@tikzborder}{#1}%
    \ALG@drawvline{\currenttextarea.north west}{\currenttextarea.south east}{#2}%
    \addtocounter{ALG@tikzborderpages\theALG@tikzborder}{-1}%
    \ifnum\value{ALG@tikzborderpages\theALG@tikzborder}>1
        \AtBeginShipoutNext{\ALG@tikzborderpage{#1}{#2}}%
    \fi
    \vspace{-0.5\baselineskip}% Compensate for the generated extra space at begin of the page. No idea why exactly this happens.
}


\def\ALG@tikzbordertext{\the\ALG@tlm}
\makeatother
% end vertical rule patch for algorithmicx



% continuation indent patch, slightly extended from https://tex.stackexchange.com/questions/78776/forced-indentation-in-algorithmicx to support multiple paragraphs in one block
\RequirePackage{etoolbox}
\makeatletter
\newlength{\ALG@continueindent}
\setlength{\ALG@continueindent}{2em}
\newcommand*{\ALG@customparshape}{\parshape 2 \leftmargin \linewidth \dimexpr\ALG@tlm+\ALG@continueindent\relax \dimexpr\linewidth+\leftmargin-\ALG@tlm-\ALG@continueindent\relax}
\newcommand*{\ALG@customparshapex}{\parshape 1 \dimexpr\ALG@tlm+\ALG@continueindent\relax \dimexpr\linewidth+\leftmargin-\ALG@tlm-\ALG@continueindent\relax}
\apptocmd{\ALG@beginblock}{\ALG@customparshape\everypar{\ALG@customparshapex}}{}{\errmessage{failed to patch}}
\makeatother
% end continuation indent patch


==> omitted-algs.tex <==
\clearpage
	\begin{algorithm}
		\caption{$\LearnCMTA(T,C,H,B)$.}\label{alg:cstar}\label{alg:learn}
		\begin{algorithmic}[1]
			\State  Initialize $B\gets\emptyset,~T\gets\emptyset,~C\gets\{\context\}$ 
			\State $\Complete(T,C,H,B,\Sigma_0)$			
			\While{true}
			\State $\mathcal{A}\gets \ExtractCMTA(T,C,H,B)$
			\State $t\gets\seq(\mathcal{A})$
			\If{$t$ is null}
			\State \Return $\mathcal{A}$
			\EndIf
			\State $\Complete(T,C,H,B,  \pref(t))$
			\EndWhile
		\end{algorithmic}
	\end{algorithm}
\clearpage
{
	\begin{algorithm}
		\caption{$\Close(T,C,H,B)$.}\label{proc:close}
		\begin{algorithmic}[1]
			\While{$\exists t\in \Sigma(T)$ s.t. $H[t]$ is co-linearly independent from $T$}
			\State $B\gets B\cup \{t\}$
			\State $T\gets T\cup \{t\}$
			\EndWhile
		\end{algorithmic}
	\end{algorithm}
}
\clearpage
{
	\begin{algorithm}
		\caption{$\Consistent(T,C,H,B)$}\label{proc:consistent}
		\begin{algorithmic}[1]
			\For{$t\in T$ s.t. $H[t]=\overline{0}$}
			\For{$c\in\Sigma(T,\context),c'\in C$}
			\If{$H[\contextConcat{c'}{c[t]}]\neq \overline{0}$}
			\State $C\gets C \cup\{\contextConcat{c}{c'}\}$
			\EndIf
			\EndFor
			\EndFor
			\For{$t_1,t_2\in T$ s.t. $ t_1\treesColin{\alpha}{H} t_2$}
			\For{$c\in\Sigma(T,\context),c'\in C$}
			\If{$H[{c'}][\contextConcat{c}{t_1}]\neq \alpha H[{c'}][{\contextConcat{c}{t_2}}]$}
			\State $C\gets C \cup\{\contextConcat{c}{c'}\}$
			\EndIf
			\EndFor
			\EndFor
		\end{algorithmic}
	\end{algorithm}
}
\clearpage
{
	\begin{algorithm}
		\caption{$\Complete(T,C,H,B,S)$.}\label{proc:complete}
		\begin{algorithmic}[1]
			\State  $T\gets T \cup S$ 
			\While{$(T,C,H,B)$ is not closed or not consistent}
			\State $\Close(T,C,H,B)$
			\State $\Consistent(T,C,H,B)$
			\EndWhile
		\end{algorithmic}
	\end{algorithm}
} 


\clearpage

\commentout{
	\begin{algorithm}
		\caption{$\Consistent(T,C,H,B)$}\label{proc:consistent}
		\begin{algorithmic}[1]
			\For{$t\in T$ s.t. $H[t]=\overline{0}$}
			\For{$t'\in\Sigma(T,t)$}
			\For{$c\in C$}
			\If{$H[\contextConcat{c}{t'}]\neq \overline{0}$}
			\State $C\gets C \cup\{\contextConcat{c}{c_t'}\}$
			\EndIf
			\EndFor
			\EndFor
			\EndFor
			\For{$t_1,t_2\in T$ s.t. $ t_1\treesColin{\alpha}{H} t_2$}
			\For{$c\in\Sigma(T,\context),c'\in C$}
			\If{$H[{c'}][\contextConcat{c}{t_1}]\neq \alpha H[{c'}][{\contextConcat{c}{t_2}}]$}
			\State $C\gets C \cup\{\contextConcat{c}{c'}\}$
			\EndIf
			\EndFor
			\EndFor
		\end{algorithmic}
	\end{algorithm}
}

\clearpage


\clearpage 

\begin{algorithm}[H]\label{alg:cstarExtract}
\caption{Extract CMTA}
\begin{algorithmic}[1]
\State $d\gets |B|$
\For {$0\leq k\leq p$}
\For {$\sigma\in \Sigma_{(k)}$}
\For {$(i_{1},i_{2},\dots,i_{k})\in \{1,2,\dots,d\}^{k}$}
\State Let $t=\sigma(b_{i_{1}},b_{i_{2}},\dots,b_{i_{k}})$
\If {$H[t]=\bar{0}$}
\For {$1\leq j\leq d$}
\State $\sigma^{j}_{i_{1},i_{2},\dots,i_{k}}\gets 0$
\EndFor
\Else
\State Let $b_{i}\in B,\alpha\in\mathbb{R}$ be s.t. $t_{i_{1},i_{2},\dots,i_{k}}\treesColin{\alpha}{H} b_{i}$
\For {$1\leq j\leq d$}
\If {$j=i$}
\State $\sigma^{j}_{i_{1},i_{2},\dots,i_{k}}\gets\alpha$
\Else
\State $\sigma^{j}_{i_{1},i_{2},\dots,i_{k}}\gets 0$
\EndIf
\EndFor
\EndIf
\EndFor
\State Let $\mu_{\sigma}$ be the $d\times d^{k}$ matrix obtained from the respective coefficients.
\EndFor
\EndFor
\For {$1\leq j\leq d$}
\State $\lambda[j]\gets H(\context,b_{j})$
\EndFor
\State \Return $\mathcal{A}=(\Sigma,\mathbb{R},d,\mu,\lambda)$
\end{algorithmic}
\end{algorithm}

\clearpage

\begin{figure}
\centering
	\scalebox{.9}{\small{
	\begin{tabular}{l@{\qquad\qquad}l}
$M_\eta = \begin{pmatrix}
c^1_{{111}} & c^1_{{112}}& c^1_{{121}} & c^1_{{122}} & c^1_{{211}} & c^1_{{212}}& c^1_{{221}} & c^1_{{222}} \\[1mm]
c^2_{{111}} & c^2_{{112}}& c^2_{{121}} & c^2_{{122}} & c^2_{{211}} & c^2_{{212}}& c^2_{{221}} & c^2_{{222}} 
\end{pmatrix}$
&
$P_{xyz} =  \begin{pmatrix}
x_1 y_1 z_1 \\
x_1 y_1 z_2 \\
x_1 y_2 z_1 \\
%x_1 y_2 z_2 \\
%x_2 y_1 z_1 \\
%x_2 y_1 z_2 \\
%x_2 y_2 z_1 \\
\ldots \\
x_2 y_2 z_2 \\
\end{pmatrix}$
\end{tabular}
}}\vspace{-2mm}
\end{figure} 
\clearpage
	\begin{tabular}{c@{\qquad}c@{\qquad}c}
	            \raisebox{1.2\height}{
	            \begin{tabular}{@{}c@{}}
	            \raisebox{0.9\height}{
				$\lambda=\begin{pmatrix}1\\0
				\end{pmatrix}$ 
				$\mu_{a}= \begin{pmatrix}1\\1
				\end{pmatrix}$ }
				\\
	            $\mu_{b} = \begin{pmatrix}
				0 & 1 & 1 & 0 \\[1mm]
				0 & 0 & 0 & 1 
				\end{pmatrix}$
	            \end{tabular}}&
				\begin{tikzpicture}
				\tikzstyle{myarrow}=[line width=.5mm,draw=#1,-triangle 45,postaction={draw, line width=4mm, shorten >=5mm, -}]
				\node[shape=circle, draw=none] (a1) at (2, 1) {$a$};
				\node[] (a1v) at (3.5, 1) {${\biword{1}{1}}$};
				\node[] (a2v) at (1.5, 1) {${\biword{1}{1}}$};
				\node[shape=circle, draw=none]  (a2) at (3, 1) {$a$};
				\node[shape=circle, draw=none] (a3) at (3.65, 2.0) {$a$};
				\node[] (a3v) at (4.10, 2.0) {${\biword{1}{1}}$};
				\node[shape=circle, draw=none]  (b1) at (2.5, 2.0) {$b$};
				\node[] (a3v) at (2.0, 2.0) {${\biword{2}{1}}$};
				\node[shape=circle, draw=none]  (b2) at (3, 3) {$b$};
				\node[] (b2v) at (2.5, 3) {${\biword{3}{1}}$};
				\draw (b2) -- (a3);
				\draw (b2) -- (b1);
				\draw (b1) -- (a1);
				\draw (b1) -- (a2);
				\end{tikzpicture}&
				\raisebox{0.75\height}{
				\scalebox{0.75}{
				\begin{tabular}{@{}c@{}}
				\begin{tikzpicture}
				\tikzstyle{myarrow}=[line width=.5mm,draw=#1,-triangle 45,postaction={draw, line width=4mm, shorten >=5mm, -}]
				\node[shape=circle, draw=none] (a1) at (2, 0.66) {$a$};
				\node[shape=circle, draw=none]  (a2) at (3, 0.66) {$b$};
				\node[shape=circle, draw=none] (a3) at (3.65, 1.33) {$c$};
				\node[shape=circle, draw=none]  (b1) at (2.5, 1.33) {$d$};
				\node[shape=circle, draw=none]  (b2) at (3, 2) {$e$};
				\draw (b2) -- (a3);
				\draw (b2) -- (b1);
				\draw (b1) -- (a1);
				\draw (b1) -- (a2);
				\end{tikzpicture}\\
				\begin{tikzpicture}
				\tikzstyle{myarrow}=[line width=.5mm,draw=#1,-triangle 45,postaction={draw, line width=4mm, shorten >=5mm, -}]
				\node[shape=circle, draw=none] (a1) at (2, 0.66) {$?$};
				\node[shape=circle, draw=none]  (a2) at (3, 0.66) {$?$};
				\node[shape=circle, draw=none] (a3) at (3.65, 1.33) {$?$};
				\node[shape=circle, draw=none]  (b1) at (2.5, 1.33) {$?$};
				\node[shape=circle, draw=none]  (b2) at (3, 2) {$?$};
				\draw (b2) -- (a3);
				\draw (b2) -- (b1);
				\draw (b1) -- (a1);
				\draw (b1) -- (a2);
				\end{tikzpicture}
				\end{tabular}}}
				\\
				(I.i)&(I.ii)&(II)
	\end{tabular}
\clearpage
\newcommand{\startprod}[1]{$#1\rightarrow$}
\newcommand{\derivation}[3]{\hlc[yellow!#3]{#1 [#2]}$\:\mid\:$}
\newcommand{\lastderivation}[3]{\hlc[yellow!#3]{#1 [#2]}}
\newcommand{\spacing}[0]{\:}
\newcommand{\cfgopt}[0]{\,|\,}
\newcommand{\scalefactor}{0.9}
\newcommand{\hlc}[2][yellow]{{%
    \colorlet{foo}{#1}%
    \sethlcolor{foo}\hl{#2}}%
}
\scalebox{\scalefactor}{
\:\:\:\startprod{S} \makebox[8.45cm]{\derivation{R N7}{0.456}{45}\derivation{R N3}{0.185}{18}\derivation{C N1}{0.137}{13}\derivation{N7 R}{0.078}{7}}
}
\scalebox{\scalefactor}{
\makebox[11.25cm]{\derivation{R N6}{0.053}{5}\derivation{N1 C}{0.034}{3}\derivation{N5 R}{0.028}{2}\derivation{N6 R}{0.013}{1}}
}
\scalebox{\scalefactor}{
\makebox[6.72cm]{\derivation{N3 R}{0.012}{1}\lastderivation{R N5}{0.004}{0}}
}

\scalebox{\scalefactor}{
\startprod{N1} \derivation{R N2}{0.640}{64}\derivation{N2 R}{0.160}{16}\derivation{R N4}{0.160}{16}\lastderivation{N4 R}{0.040}{4}
}

\scalebox{\scalefactor}{
\startprod{N2} \lastderivation{A B}{1.000}{100} \startprod{N3} \lastderivation{C N2}{1.000}{100}  \startprod{N4} \lastderivation{B A}{1.000}{100}
}

\scalebox{\scalefactor}{
\startprod{N5} \lastderivation{N4 C}{1.000}{100} \startprod{N6} \derivation{C N4}{0.882}{88}\derivation{N8 A}{0.095}{9}\lastderivation{A N8}{0.024}{2}
}

\scalebox{\scalefactor}{
\startprod{N7} \lastderivation{N2 C}{1.000}{100} \startprod{N8} \derivation{B C}{0.800}{80}\lastderivation{C B}{0.200}{20}
}

\scalebox{\scalefactor}{
\:\:\:\startprod{R} \lastderivation{AcrR}{1.000}{100} \startprod{A} \lastderivation{AcrA}{1.000}{100} \startprod{B} \lastderivation{AcrB}{1.000}{100}
}

\scalebox{\scalefactor}{
\:\:\:\startprod{C} \lastderivation{TolC}{1.000}{100}
}

\begin{tikzpicture}
\node[draw=none] (t1) at (0, 0) {
\scalebox{0.6}{
\begin{tikzpicture}
\tikzstyle{myarrow}=[line width=3mm,draw=#1]
\draw [myarrow={cyan}](1.2,3.5)--(-0,3.5);
\draw [myarrow={red}](1.4,3.5)--(2.6,3.5);
\draw [myarrow={green}](3,3.5)--(4.2,3.5); 
\draw [myarrow={yellow}](4.5,3.5)--(5.7,3.5); 
\node[draw=none] (S) at (2.5, 6) {$S$};
\node[draw=none] (R) at (0.6, 5) {$R$};
\node[draw=none] (A) at (2, 4.25) {$A$};
\node[draw=none] (B) at (3.5, 4.25) {$B$};
\node[draw=none] (C) at (5, 4.25) {$C$};
\node[draw=none] (N2) at (2.7, 5) {$N_{2}$};
\node[draw=none] (N7) at (3.7, 5.5) {$N_{7}$};
\node[draw=none] (acrA) at (2,3.5) {AcrA};
\node[draw=none] (acrB) at (3.5,3.5) {AcrB};
\node[draw=none] (tolC) at (5,3.5) {TolC};
\node[draw=none] (acrR) at (0.6,3.5) {AcrR};
\draw (S) -- (N7);
\draw (S) -- (R);
\draw (N7) -- (N2);
\draw (N7) -- (C);
\draw (N2) -- (A);
\draw (N2) -- (B);
\draw (R) -- (acrR);
\draw (A) -- (acrA);
\draw (B) -- (acrB);
\draw (C) -- (tolC);
\end{tikzpicture}}};
\node[draw=none] (t2) at (5, 0) {\scalebox{0.6}{
\begin{tikzpicture}
\tikzstyle{myarrow}=[line width=3mm,draw=#1]
\draw [myarrow={cyan}](3,3.75)--(4.2,3.75); 
\draw [myarrow={red}](1.4,3.75)--(2.6,3.75);
\draw [myarrow={green}](1.2,3.75)--(-0,3.75);
\draw [myarrow={yellow}](4.5,3.75)--(5.7,3.75); 
\node[draw=none] (S) at (3.5, 6.3) {$S$};
%\node[draw=none] (Ps) at (3.5, 7) {$0.522$}
\node[draw=none] (N1) at (2.5, 5.75) {$N_{1}$};
%\node[draw=none] (P1) at (0.5, 4.5) {$1.000$}
\node[draw=none] (A) at (2, 4.5) {$A$};
%\node[draw=none] (P2) at (2.2, 3.25) {$1.000$}
\node[draw=none] (B) at (0.5, 4.5) {$B$};
\node[draw=none] (R) at (3.5, 5) {$R$};
%\node[draw=none] (P3) at (4.2, 3.25) {$1.000$}
\node[draw=none] (N4) at (1.25, 5) {$N_{4}$};
\node[draw=none] (C) at (5, 5) {$C$};
\node[draw=none] (acrA) at (2,3.75) {AcrA};
\node[draw=none] (acrB) at (0.5,3.75) {AcrB};
\node[draw=none] (tolC) at (5,3.75) {TolC};
\node[draw=none] (acrR) at (3.5,3.75) {AcrR};

\draw (S) -- (N1);
\draw (S) -- (C);
\draw (N1) -- (N4);
\draw (N1) -- (R);
\draw (N4) -- (B);
\draw (N4) -- (A);
\draw (R) -- (acrR);
\draw (A) -- (acrA);
\draw (B) -- (acrB);
\draw (C) -- (tolC);
\end{tikzpicture}}};

\node[draw=none] (t3) at (2.5,0.2) {\scalebox{0.55}{\begin{tikzpicture}
\tikzstyle{myarrow}=[line width=3mm,draw=#1]
\draw [myarrow={cyan}](1,1.5)--(1,2.5);
\draw [myarrow={red}](0,1.5)--(0,2.5);
\draw [myarrow={green}](2,1.5)--(2,2.5);
\draw [myarrow={yellow}](3,1.5)--(3,2.5); 
\node[shape=circle,draw=black] (P) at (1.5, 3.5) {};
\node[draw=none, rotate=90] (acrA) at (0,2) {AcrA};
\node[draw=none, rotate=90] (acrB) at (2,2) {AcrB};
\node[draw=none, rotate=90] (tolC) at (3,2) {TolC};
\node[draw=none, rotate=90] (acrR) at (1,2) {AcrR};

\draw (P) -- (acrR);
\draw (P) -- (acrA);
\draw (P) -- (acrB);
\draw (P) -- (tolC);
\end{tikzpicture}}};
\end{tikzpicture}

==> proof_posrank-for-HM.tex <==
\textbf{Theorem~\ref{thm:posrank-for-HM}} (page~\pageref{thm:posrank-for-HM}) states the following
\begin{center}
	Let $\aut{M}=(\Sigma,\K,d,\mu,\lambda)$ be a PMTA, \\
	and let $\hm{H}$ be the Hankel Matrix of $\mathcal{M}$. \\
	Then $\rank(\hm{H})\leq d$.
\end{center} 
\begin{proof}[Proof of Theorem~\ref{thm:posrank-for-HM}]\label{proof:thm:posrank-for-HM}
	Let $\mu_\sigma$ be the $k$-linear function the MTA $\aut{M}$ associates with $\sigma \in \Sigma_k$.
	For every $\sigma\in \Sigma_k$ for $k>0$,  with every $1\leq i \leq k$ we can associae a $(k-1)$-linear function $\mu_\sigma^i$ from $\V^{k-1}$ to $\V\rightarrow \V$ defined so that 
	for every $\textbf{v}_1,\ldots,\textbf{v}_k\in \V$ we have
	$$\mu_\sigma(\textbf{v}_1,\ldots,\textbf{v}_k)=\textbf{v}_i \cdot \mu_\sigma^i(\textbf{v}_1,\ldots,\textbf{v}_{i-1},\textbf{v}_{i+1},\ldots\textbf{v}_k)$$
	
	Given a context $c\in \trees_\$(F)$ we can associate with it a linear transformation from $\V$ to $\V$ defined recursively as follows, where
	we use $\nu_c$, a $d\times d$ matrix over $ \K$ to define the respective linear transformation.
	If $c = \context$ then $\nu_c$ is the identity matrix. Otherwise, $c=\sigma(t_1,\ldots,t_{j-1},c',t_{j+1},\ldots,t_k)$ for some context $c'\in\trees_\context(\F)$.
	In this case $$\nu_c = \nu_{c'} \cdot \mu_\sigma^j(\mu(t_1),\ldots,\mu(t_{j-1}),\mu(t_{j+1}),\ldots,\mu(t_k)).$$
	Note that $\mu(t\cdot c)=\mu(t)\nu_c$.
	
	
	
	Let $t_0,t_1,t_2,\ldots$ be an anumeration of all trees in $\trees(\Sigma)$.
	Let $c_0,c_1,c_2,\ldots$ be an enmueration of all contexts in $\trees_\context(\Sigma)$.
	Let $M_{rows}$ be a $\infty\times d$ matrix such that $M_{rows}(t_i,\ell)= \mu(t_i)[\ell]$ for $\ell\in\{1,\ldots,d\}$ and $t_i$ in the respective enumeration. 
	Let $M_{cols}$ be a $d \times \infty$ matrix such that $M_{cols}(\ell,c_j)= \nu_{c_j}[\ell]$ for $\ell\in\{1,\ldots,d\}$ and $c_j$ in the respective enumeration. 
	Let $M = M_{rows} M_{cols}$. Then $M(i,j)=\sum_{1\leq \ell \leq d} \, \mu(t_i)[\ell]\,\nu_{c_j}[\ell] = \mu(t_i)\cdot \nu_{c_j}= \mu(t_i\cdot c_j)$. 	
	
	Therefore, if $H$ is the Hankel Matrix of $\aut{M}$ then $H(i,j)=\lambda M(i,j)$.
	By~\cite[Lemma 2.3]{cohen1993nonnegative} the positive rank of a matrix is bounded by its smallest dimension, thus $\prank(M_{rows})\leq d$ and $\prank(M_{cols})\leq d$.
	By~\cite[Lemma 2.6]{cohen1993nonnegative} $\prank(AB)\leq\min\{\prank(A),\prank(B)\}$ hence the positive rank of $M$ and $H$ is also bounded by $d$.
\end{proof}


==> response.tex <==
We thank the reviewers for the time they invested in reviewing the paper, and for their valuable comments. Below are our responses to the critical comments and questions of the reviewers. 


Reviewer #1:
-----------

R#1 Q11:
-	As mentioned in the intro PCFGs cannot be polynomially learned using MQ and EQ, therefore some restriction must be applied. The restriction to work with structured strings has been proposed before for the more restricted cases of tree automata and unweighted CFGs.  

-	As for the unambiguity requirement, it follows from Gray and Harrison [6] that every context-free language has a reversible CFG. In Lemma B.5 (in the supplementary material) we've shown that reversible CFGs are equivalent to SUCFGs. Therefore the unambiguity requirement, doesn't restrict the class of studied phenomena. 

R#1 Q13:
    Correct, thanks for pointing this out.


Reviewer #3:
-----------

R#3 Q11,  Q13:
    see R#1 Q11.
    

R#3 Q12:
    Pseudo-code for both methods is available in the supplementary material. (Algorithms 1, 2 Section B.3, line 911)

Reviewer #5:
-----------

R#5 Q7, Q8:
    The code and data-sets that were used in the demonstration part were provided with the supplementary material (PCFGLearner.zip).

R#5 Q6 Q11 Q13:
-	The last section was not intended to provide empirical results,  but rather it is given as a demonstration for the usefulness of the proposed algorithm in learning genomic data. The proposed algorithm is the first to solve the problem defined in this paper. Hence there are no obvious tools and datasets yet to compare against. 
-   The 1st example in the section does show that the state-of-the-art model used to represent a grammar for this type of genomic data is much inferior in terms of specificity. 
-   The 2nd example shows that our algorithm can be applied to genomic data with duplications (that derive infinite languages), and cannot be modeled by PQ-trees.

R#5 Q12:
Thanks for pointing out to these references, we will read them carefully and compare if possible.

Reviewer #6:
-----------

R#6 Q5:
	Given the page limit, and the technical complexity of the theoretical contribution, we did our best to distribute the explanatory information between the main paper and the supplementary material. 

R#6 Q6, Q11-R3:
  addressed in R#5 Q6 Q11 Q13:
  
R#6 Q7, Q8: The code and data-sets that were used in the demonstration part were provided with the supplementary material (PCFGLearner.zip).

R#6 Q11 R1:
    We will clarify the high level contribution. The bottom line is that we have identified a non-trivial sub-class of PCFGs for which query learning can be done in polynomial time. We provide the required definitions, explanations why the class is not learnable via state-of-the-art approaches, an algorithm and a theoretical proof for its correctness and time and query complexity. We provide motivation for the usefulness of the algorithm in the context of inferring gene-cluster grammars.
    
R#6 Q11 R2:
 PCFG's can be used to model gene cluster grammars, and as mentioned in the introduction (138-145) gene cluster grammars can be used for various practical applications in computational biology. "The  gene  grammar  corresponding to a given gene cluster describes its hierarchical inner  structure  and  the  relations  between  instances  of  the cluster succinctly; assists in predicting the functional association between the genes in the cluster; provides insights into the evolutionary history of the cluster; aids in filtering meaningful from apparently meaningless clusters; and provides a natural and meaningful way of visualizing complex clusters."

R#6 Q11 R4,:
	Working with the space restriction of the CFP guidelines, the supplementary material contains all missing proofs, as well as reproducibility details on the demonstration. AAAI and similar conferences have been known to give some stage to theoretical results of such nature (see e.g. [1,2,3,4]). 

R#6 Q12:

323: Both mu and lambda should be non-negative; Thanks we will clarify.

431-432 and 444 until section 4.1 - These are great questions. 
a. Even for the word case, the problem of converting an MA of a positive word-series to an equivalent PMA seems hard. In the algebraic sense, it is similar to the question of finding a similar non-negative matrix. This question is interesting in many other applications, and is known to be hard. (The algebraic question seeks for a similar matrix of the same dimension, and it seems to us that the relaxation to allow matrices of higher dimensions makes the problem harder.)
b. Proposition 4.2 shows that there is a language, that can be recognized by a PMTA, but the M* algorithm cannot find it. This is since any finite subset of row-vectors from the Hankel Matrix, doesn't positively-span the entire infinite matrix. M* will fail, since it works by looking for a base (subset of row-vectors) that linearly spans the entire matrix. Since there is no such base that positively spans the matrix, if M* would terminate, it will not return a positive base.

466-467: Thanks for another great question, as we show in Lemma B.5 in the supplementary material, a CFG is invertible iff it is structurally unambiguous. [6] proved that for any context-free language L, there is an invertible grammar G such that L(G) = L.  This result can be easily lifted to PCFGs. This shows that there aren't inherently structurally ambiguous languages.

476: Thanks again, the proof should start with a sentence saying that since that grammar is structurally unambiguous, there is a 1-to-1 correspondence between tagged and skeletal trees. Therefore a row in the Hankel matrix of an SUPCFG corresponds to a tagged tree.

507-510: The term co-linear is used, since two rows of the Hankel matrix are considered equivalent if they are co-linear. Two vectors are co-linear if they are parallel (i.e their cross-product is the 0 vector).

636: Yes, it should be (1/2)^n

R#6 Q13.Q2
-	Glad you asked. A query learning algorithm for PDFAs was proposed in [5]. However, that work did not utilize the fact that two rows of the Hankel matrix can be correspond to the same state of the PDFAs, if they are co-linear. Instead their learning algorithm separates two rows if the difference between them exceeds a given threshold t. Consider a language generated by a PDFA with one state over one letter with a self loop with probability p. For a long word, say of length k, and a similarity constant t that is less than p^k-p^{k-1}, the PDFA inferred by their algorithm will have k states, whereas using our algorithm the inferred PDFA will be of size one.   

R#6 Q13.Q1 
-  As can be observed from answer R#6 Q13.Q2, even for the simpler case of word languages, the relevant theory missed the compression that can be achieved by considering co-linear dependencies in the Hankel matrix. This shows that our algorithm not only addresses the more complex setting of tree languages, but also does so by providing more succinct automata.

R#6 Q13.Q3
See R#5 Q6 Q11 Q13:

R#6 Q13.Q4
Yes, this is a good point, it would be interesting to compare the results of the simpler case of the word-level version of our algorithm, to existing PDFA learning algorithms.


Thanks again for the thorough reading of our paper.

[1] Sebastian Berndt, Maciej Liskiewicz, Matthias Lutter, and Rudiger Reischuk: Learning Residual Alternating Automata. AAAI 2017. 
[2] Benedikt Bollig, Peter Habermehl, Carsten Kern, Martin Leucker: Angluin-Style Learning of NFA. IJCAI 2009.
[3] Dana Angluin, Sarah Eisenstat, Dana Fisman: Learning Regular Languages via Alternating Automata. IJCAI 2015
[4] Jakub Michaliszy and Jan Otop: Learning Deterministic Automata on Infinite Words. ECAI 2020
[5] Weiss, Goldberg, Yahav: Learning Deterministic Weighted Automata with Queries and Counterexamples. NeurIPS 2019.
[6] Gray, Harrison: On the Covering and Reduction Problems for Context-Free Grammars. JACM 1972.

------------------------------------------------------------

1.Toning down the demonstration section. Making clear that it is only a proof-of-concept:

Move the description of the demonstration from the introduction to the demo section. In the intro, write:
As a proof-of-concept, in Section (DEMO), we exemplify our algorithm by applying it to a small data-set of genomic data.


2.Maybe remove from the demo:
lines 592-598
